Adaptive pointwise density estimation under local differential privacy

We consider the estimation of a density at a fixed point under a local differential privacy constraint, where the observations are anonymised before being available for statistical inference. We propose both a privatised version of a projection density estimator as well as a kernel density estimator and derive their minimax rates under a privacy constraint. There is a twofold deterioration of the minimax rates due to the anonymisation, which we show to be unavoidable by providing lower bounds. In both estimation procedures a tuning parameter has to be chosen. We suggest a variant of the classical Goldenshluger-Lepski method for choosing the bandwidth and the cut-off dimension, respectively, and analyse its performance. It provides adaptive minimax-optimal (up to log-factors) estimators. We discuss in detail how the lower and upper bound depend on the privacy constraints, which in turn is reflected by a modification of the adaptive method.

==> packages.tex <==
% 
\usepackage[ngerman,english]{babel}
\RequirePackage{ucs}
\RequirePackage[utf8x]{inputenc}
%
% zeige labels am rand an.
%\usepackage[notref,notcite]{showkeys} 
%%  aendere Anzeige der labels         
% \renewcommand{\showkeyslabelformat}[1]{%
%	\mbox{\dg \normalfont\tiny\ttfamily#1}}
%%
%
%\usepackage{lmodern} % font: Latin Modern
%\usepackage[right = 2cm, top=2.5cm, bottom=2.5cm,left=2cm]{geometry}
%
%
%
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{thmtools}
\usepackage{mathtools}
\usepackage{amsfonts}
\usepackage{float}
\usepackage{lmodern} % font: Latin Modern
\usepackage[right = 2.5cm, top=2.5cm, bottom=2.5cm,left=2.5cm]{geometry}
\usepackage{appendix}
\usepackage{chngcntr}
%\pgfplotsset{compat=1.13}
%
%==========================================
\RequirePackage{amsthm,amsmath}
\RequirePackage{amssymb,amstext}
\RequirePackage{amsfonts,stmaryrd}
\RequirePackage{amsbsy} 
\RequirePackage{mathrsfs}
\RequirePackage{bm}
\RequirePackage{bbm}
\RequirePackage{aliascnt,ifthen}
\RequirePackage{graphicx}
\RequirePackage{color,calc}
\RequirePackage{url}
\RequirePackage{verbatim}

\RequirePackage{relsize}

\usepackage[pdfpagemode=UseOutlines ,plainpages=false,
%hypertexnames=false ,pdfpagelabels=TRUE ,
hyperindex=true,colorlinks=true]{hyperref}
	\makeatletter
	\Hy@breaklinkstrue
	\makeatother

\definecolor{darkred}{rgb}{0.6,0,0.1}
\definecolor{darkgreen}{rgb}{0,0.5,0}
\definecolor{darkblue}{rgb}{0,0,0.5}

\hypersetup{colorlinks ,linkcolor=gray ,filecolor=darkgreen,  urlcolor=blue ,citecolor=black}

\RequirePackage{paralist}

% BIBLIOGRAPHY
\usepackage{natbib}
\usepackage{hypernat}
\renewcommand{\cite}{\citet}
\bibliographystyle{abbrvnat}

%==========================================
% Packages Sandra
%==========================================
\usepackage{enumitem} % advanced enumeration
\usepackage{graphicx} % for including graphics
\usepackage{dsfont} % indicator function \mathds{1}
\usepackage{tikz,pgfplots} % tikz pgf: advanced drawing
\usetikzlibrary{shapes.geometric, arrows.meta, calc, positioning, shapes.multipart}
\usepackage[framemethod=TikZ]{mdframed}
\usepackage{ifthen}
\usepackage{supertabular} % tables with pagebreaks
\usepackage{booktabs}  % nicer tables
\usepackage{cases}
\usepackage{xcolor}
\usepackage{blindtext}
\usepackage{multirow}
\usepackage{textcmds}

\usepackage{cleveref}
\crefname{definition}{\color{\colde}Definition}{\color{\colde}Definitions}
\crefname{figure}{\color{\colde}Figure}{\color{\colde}Figures}
\crefname{lemma}{\color{\colre}Lemma}{\color{\colre}Lemmata}
\crefname{example}{\color{\colre}Example}{\color{\colre}Examples}
\crefname{proposition}{\color{\colre}Proposition}{\color{\colre}Propositions}
\crefname{reminder}{\color{\colrem}Reminder}{\color{\colrem}Reminder}
\crefname{theorem}{\color{\colre}Theorem}{\color{\colre}Theorems}
\crefname{corollary}{\color{\colre}Corollary}{\color{\colre}Corollaries}
\crefname{remark}{\color{\colrem}Remark}{\color{\colrem}Remarks}
\crefname{assumption}{\color{\colre}Assumption}{\color{\colde}Assumptions}
\crefname{illustration}{\color{\colil}Illustration}{\color{\colil}Illustrations}
\crefname{section}{\color{\colre}Section}{\color{\colre}Sections}
\crefname{appendix}{\color{\colre}Appendix}{\color{\colre}Appendices}
\crefname{chapter}{\color{\colre}Chapter}{\color{\colre}Chapters}
\numberwithin{equation}{section} 


%%%%% TIKZ
\usetikzlibrary{shapes.misc}
\tikzset{cross/.style={cross out, draw=black, fill=none, minimum size=2*(#1-\pgflinewidth), inner sep=0pt, outer sep=0pt}, cross/.default={2pt}}
\usetikzlibrary{patterns, shapes,positioning,decorations.pathmorphing}
\makeatletter
\pgfdeclarepatternformonly[\GridSize]{MyGrid}{\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{4pt}{4pt}}{\pgfqpoint{\GridSize}{\GridSize}}%
{
	\pgfsetcolor{\tikz@pattern@color}
	\pgfsetlinewidth{0.3pt}
	\pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
	\pgfpathlineto{\pgfqpoint{\GridSize + 0.1pt}{\GridSize + 0.1pt}}
	%	\pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
	%	\pgfpathlineto{\pgfqpoint{0pt}{3.1pt}}
	%	\pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
	%	\pgfpathlineto{\pgfqpoint{3.1pt}{0pt}}
	\pgfusepath{stroke}
}
\makeatother

\newdimen\GridSize
\tikzset{
	GridSize/.code={\GridSize=#1},
	GridSize=3pt
}
\tikzstyle{startstop} = [rectangle, thick, rounded corners,   minimum width = 3cm, minimum height = 1cm, draw = gray, fill=blue!10]
\tikzstyle{startstop2} = [rectangle, thick, rounded corners,   minimum width = 3cm, minimum height = 1cm, draw = gray, fill=green!10]
\tikzstyle{startstop3} = [cloud, cloud, draw, align=left, cloud puffs=20,cloud puff arc=110, aspect=3, inner sep=0mm, draw = gray, fill=orange!10]
\tikzstyle{arrow5} = [ultra thick, dotted]
\tikzset{ellip/.style={ellipse,thin, dotted,draw, fill=gray!05}}
%
\usetikzlibrary{decorations.text}


\usepackage{textcmds}

%%%
% hfill for align
\makeatletter
\newcommand{\pushright}[1]{\ifmeasuring@#1\else\omit\hfill$\displaystyle#1$\fi\ignorespaces}
\newcommand{\pushleft}[1]{\ifmeasuring@#1\else\omit$\displaystyle#1$\hfill\fi\ignorespaces}
\makeatother
%
\renewcommand{\labelitemi}{$\color{gray}\blacktriangleright$}

\global\mdfdefinestyle{test}{
	linecolor=gray!20!white, linewidth=2pt,%
	innertopmargin=0pt,%
	backgroundcolor=gray!20!white
}

\global\mdfdefinestyle{object}{
	linecolor=green!50!black, linewidth=1pt,%
	innertopmargin=0pt,%
	topline=false,rightline=true,bottomline=false
}
